Data fusion for efficiency gain in ATE estimation: A practical review with simulations

The integration of real-world data (RWD) and randomized controlled trials (RCT) is increasingly important for advancing causal inference in scientific research. This combination holds great promise for enhancing the efficiency of causal effect estimation, offering benefits such as reduced trial participant numbers and expedited drug access for patients. Despite the availability of numerous data fusion methods, selecting the most appropriate one for a specific research question remains challenging. This paper systematically reviews and compares these methods regarding their assumptions, limitations, and implementation complexities. Through simulations reflecting real-world scenarios, we identify a prevalent risk-reward trade-off across different methods. We investigate and interpret this trade-off, providing key insights into the strengths and weaknesses of various methods; thereby helping researchers navigate through the application of data fusion for improved causal inference.

==> shortcuts_v1.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Packages                                  %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage[utf8]{inputenc}
\usepackage{amsmath, amsfonts, amsthm, amssymb, bbm, bm}
\usepackage{mathrsfs}
\usepackage{centernot}
%\usepackage{euscript}
\usepackage{enumerate}
%\usepackage{calligra}
\usepackage{tabularx}
\usepackage{multicol}
\usepackage{multirow}
% \usepackage{relsize}
\usepackage[colorlinks=true,linktoc=all, allcolors=black]{hyperref}
\usepackage{setspace}
\setstretch{1.5}
\usepackage[margin=3cm]{geometry}
\usepackage[round]{natbib}
\usepackage{booktabs}
\usepackage{tikz}
\usetikzlibrary{shapes,arrows,calc}
\usepackage{algorithm} 
\usepackage{algpseudocode} 
\usepackage{authblk}
\usepackage[english]{babel} % To obtain English text with the blindtext package
\usepackage{blindtext}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Symbols                                   %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\renewcommand{\Pr}{\mathbb{P}}
%\newcommand{\E}{\scalebox{1.1}{$\mathbb{E}$}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\D}{\mathcal{D}}
\DeclareMathOperator{\Var}{Var}
\DeclareMathOperator{\Cov}{Cov}
\DeclareMathOperator{\Corr}{Corr}
\DeclareMathOperator{\ELPD}{ELPD}
\newcommand{\Ind}{\mathbbm{1}}

\newcommand{\reals}{\mathbb{R}}

\DeclareMathOperator{\expit}{expit}
\DeclareMathOperator{\logit}{logit}

\newcommand{\G}{\mathcal{G}}
\newcommand{\X}{\mathfrak{X}}
\newcommand{\M}{\mathcal{M}}

\DeclareMathOperator{\ing}{ing}
\DeclareMathOperator{\diag}{diag}

\DeclareMathOperator{\tail}{tail}
\DeclareMathOperator{\patail}{pa-tail}
\DeclareMathOperator{\distail}{dis-tail}
\DeclareMathOperator{\pa}{pa}
\DeclareMathOperator{\ch}{ch}
\DeclareMathOperator{\nei}{ne}
\DeclareMathOperator{\bd}{bd}
\DeclareMathOperator{\spo}{sp}
\DeclareMathOperator{\an}{an}
\DeclareMathOperator{\ant}{ant}
\DeclareMathOperator{\un}{un}
\DeclareMathOperator{\dir}{dir}
\DeclareMathOperator{\dec}{de}
\DeclareMathOperator{\barren}{barren}
\DeclareMathOperator{\sterile}{sterile}
\DeclareMathOperator{\dis}{dis}
\DeclareMathOperator{\nhd}{nhd}
\DeclareMathOperator{\nd}{nd}
\DeclareMathOperator{\mbl}{mb}
\DeclareMathOperator{\forb}{forb}
\DeclareMathOperator{\cn}{cn}
\DeclareMathOperator{\Bernoulli}{Bernoulli}

\DeclareMathOperator{\var}{Var}
\DeclareMathOperator{\cov}{Cov}

\DeclareMathOperator{\pre}{pre}

\DeclareMathOperator{\Do}{\it do}

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\newcommand{\cmid}{\,|\,}

\newcommand{\lrarr}{\leftrightarrow}
\newcommand{\sto}{*\!\!\to}
\newcommand{\getss}{\gets\!\!*}
\newcommand{\sun}{*\!\!-}
\newcommand{\uns}{-\!\!*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Symbols                                   %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\simiid}{\stackrel{\mbox{\tiny{i.i.d.}}}{\sim}}
\newcommand{\simap}{\stackrel{\mbox{approx}}{\sim}}

% Forms of convergence
\newcommand{\tend}{\longrightarrow}
%\newcommand{\tendD}{\xrightarrow{\mathcal{D}}}
\newcommand{\tendD}{\stackrel{\mathcal{D}}{\longrightarrow}}
\newcommand{\tendd}{\stackrel{d}{\longrightarrow}}
%\newcommand{\tendp}{\xrightarrow{p}}
\newcommand{\tendp}{\stackrel{p}{\longrightarrow}}
%\newcommand{\tendas}{\xrightarrow{\mbox{\tiny{a.s.}}}}
\newcommand{\tendas}{\stackrel{\mbox{\tiny{a.s.}}}{\longrightarrow}}
\newcommand{\tendL[1]}{\xrightarrow{L_{#1}}}

\newcommand{\ntend}{\nrightarrow}
\newcommand{\ntendD}{\centernot{\xrightarrow{\mathcal{D}}}}
\newcommand{\ntendp}{\centernot{\xrightarrow{\mathbb{P}}}}
\newcommand{\ntendas}{\centernot{\xrightarrow{\mbox{\tiny{a.s.}}}}}
\newcommand{\ntendL[1]}{\centernot{\xrightarrow{L_{#1}}}}

\newcommand{\eqD}{\stackrel{\mathcal{D}}{=}}
\newcommand{\eqas}{\stackrel{\mbox{\tiny\rm a.s.}}{=}}

\newcommand{\T[1]}{{#1}^T}

\newcommand\indep{\protect\mathpalette{\protect\independenT}{\perp}}
\def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern2mu{#1#2}}}

%\newcommand{\nindep}{\indep\!\!\!\!\!\!\setminus\;\;}
\newcommand{\nindep}{\centernot{\indep}}

\newcommand{\CI}[3]{#1 \indep #2 \; | \; #3}
\newcommand{\GS}[3]{#1 \perp #2 \; | \; #3}

\newcommand{\rbow}{\mathbin{\begin{tikzpicture}[baseline] 
\draw[<->] (0pt,.3ex) -- (2ex,.3ex);
\draw[->] (0pt,1ex) -- (2ex,1ex);
\end{tikzpicture}}}

\newcommand{\lbow}{\mathbin{\begin{tikzpicture}[baseline] 
\draw[<->] (0pt,.3ex) -- (2ex,.3ex);
\draw[<-] (0pt,1ex) -- (2ex,1ex);
\end{tikzpicture}}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Theorems                                  %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\theoremstyle{plain}
\newtheorem{lem}{Lemma}[section]
\newtheorem{thm}[lem]{Theorem}
\newtheorem{prop}[lem]{Proposition}
\newtheorem{cor}[lem]{Corollary}
\newtheorem{conj}[lem]{Conjecture}
\theoremstyle{definition}
\newtheorem{dfn}[lem]{Definition}
%\theoremstyle{remark}
\newtheorem{rmk}[lem]{Remark}
\newtheorem{exm}[lem]{Example}
\newtheorem{alg}[lem]{Algorithm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Environments                              %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\benum}{\begin{enumerate}}
\newcommand{\eenum}{\end{enumerate}}

\newcommand{\bitem}{\begin{itemize}}
\newcommand{\eitem}{\end{itemize}}

\newcommand{\barr}{\begin{array}}
\newcommand{\earr}{\end{array}}

\newcommand{\bmat}{\begin{pmatrix}}
\newcommand{\emat}{\end{pmatrix}}

\newcommand{\blist}{\renewcommand{\labelenumi}{\textbf{\arabic{enumi}}.} \begin{enumerate}}
\newcommand{\elist}{\end{enumerate} \renewcommand{\labelenumi}{\arabic{enumi}.}}

%\newcommand{\mb}{\mathbf}
\newcommand{\bs}{\boldsymbol}

\def\bal#1\eal{\begin{align*}#1\end{align*}}

\newcommand{\stk}[2]{\mathsmaller{\begin{smallmatrix}#1 \\ #2\end{smallmatrix}}}

% Table padding
\renewcommand{\arraystretch}{1.5}

% Assumptions, Theorems and Stuff
\newtheorem{theorem}{Theorem}[section]
\newtheorem{corollary}{Corollary}[theorem]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{assumption}{Assumption}

\newcolumntype{L}{>{$}l<{$}}
\newcolumntype{C}{>{$}c<{$}}
\renewcommand{\arraystretch}{1.2}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Indents                                   %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\setlength{\parindent}{0pt}
\setlength{\parskip}{6pt}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% TikZ Commands                             %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{tikz}
\usetikzlibrary{shapes, arrows, arrows.meta, calc, positioning}


% nodes
\tikzset{nv/.style={circle, color=red, fill=red, inner sep=0.5mm}}
\tikzset{rv/.style={circle, draw, thick, minimum size=7mm, inner sep=0.5mm}}
\tikzset{fv/.style={rectangle, draw, thick, minimum size=7mm, inner sep=0.5mm}}
\tikzset{lv/.style={circle, color=red, fill=gray!30, draw, thick, minimum size=7mm, inner sep=0.5mm}}
\tikzset{rve/.style={ellipse, draw, thick, minimum size=7mm, inner sep=0.5mm}}

% nodes for slides
\tikzset{rvs/.style={circle, draw, thick, minimum size=6mm, inner sep=0.5mm}}
\tikzset{fvs/.style={rectangle, draw, thick, minimum size=6mm, inner sep=0.5mm}}
\tikzset{lvs/.style={circle, color=red, fill=gray!30, draw, thick, minimum size=6mm, inner sep=0.5mm}}
\tikzset{rves/.style={ellipse, draw, thick, minimum size=6mm, inner sep=0.5mm}}

% edges
\tikzset{deg/.style={->, very thick, color=blue}}
\tikzset{degl/.style={->, very thick, color=red}}
\tikzset{beg/.style={<->, very thick, color=red}}
%\pgfarrowsdeclare{os}{os}{}{$\circ$} 
\tikzset{cdeg/.style={{Circle[length=+2pt 2.5,width=+2pt 2.5, fill=none]}->, very thick, color=blue}}
\tikzset{cceg/.style={{Circle[length=+2pt 2.5,width=+2pt 2.5, fill=none]}-{Circle[length=+2pt 2.5,width=+2pt 2.5, fill=none]}, very thick}}
\tikzset{uceg/.style={{Circle[length=+2pt 2.5,width=+2pt 2.5, fill=none]}-, very thick}}
\tikzset{ueg/.style={very thick}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Colours                             %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\definecolor{oxblue}{RGB}{0, 33, 71}
